Toward Globally Optimal State Estimation Using Automatically Tightened Semidefinite Relaxations

In recent years, semidefinite relaxations of common optimization problems in robotics have attracted growing attention due to their ability to provide globally optimal solutions. In many cases, it was shown that specific handcrafted redundant constraints are required to obtain tight relaxations and thus global optimality. These constraints are formulation-dependent and typically identified through a lengthy manual process. Instead, the present paper suggests an automatic method to find a set of sufficient redundant constraints to obtain tightness, if they exist. We first propose an efficient feasibility check to determine if a given set of variables can lead to a tight formulation. Secondly, we show how to scale the method to problems of bigger size. At no point of the process do we have to find redundant constraints manually. We showcase the effectiveness of the approach, in simulation and on real datasets, for range-based localization and stereo-based pose estimation. Finally, we reproduce semidefinite relaxations presented in recent literature and show that our automatic method always finds a smaller set of constraints sufficient for tightness than previously considered.

==> _tables/ro_quad_dataset_errors_n100.tex <==
\begin{tabular}{lrr}
 & global $e_t$ & local $e_t$ \\
min & 0.074184 & 0.055883 \\
max & 2.467624 & 3.795707 \\
median & 0.375005 & 1.169177 \\
mean & 0.548598 & 1.358187 \\
std & 0.439795 & 1.049875 \\
\end{tabular}


==> _tables/stereo_dataset_errors_n100.tex <==
\begin{tabular}{lrrrr}
 & global $e_t$ & global $e_C$ & local $e_t$ & local $e_C$ \\
min & 0.014364 & 0.003276 & 1.952834 & 1.130370 \\
max & 0.339518 & 1.845242 & 11.650198 & 2.828427 \\
median & 0.082792 & 0.029484 & 7.700230 & 2.828355 \\
mean & 0.093914 & 0.044693 & 7.676829 & 2.778475 \\
std & 0.058125 & 0.121845 & 1.681287 & 0.224380 \\
\end{tabular}


==> bios.tex <==


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{_photos/frederike.png}}]{Frederike Dümbgen} (Member, IEEE) received the B.Sc. and M.Sc. degrees in mechanical engineering, with a minor in computational science and engineering, and the Ph.D.~degree in computer and communication sciences from École Polytechnique Fédérale de Lausanne (EPFL), Lausanne, Switzerland, in 2013, 2016, and 2021, respectively, and conducted her master’s thesis at ETH Zürich, Zurich, Switzerland. From 2024 to 2024, she was a Postdoctoral Researcher with the Robotics Institute, University of Toronto, Toronto, ON, Canada. As of May 2024, she is a Researcher with the WILLOW team, affiliated with Inria and ENS, PSL University, Paris, France. Her research interests include areas of estimation and advanced optimization for robotics.   
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{_photos/connor_bw.jpg}}]{Connor Holmes} (Student Member, IEEE) received the B.A.Sc.~degree in engineering science, in 2014, and the M.A.Sc.~degree in electrical and computer engineering, in 2016, from the University of Toronto, Toronto, ON, Canada, where he is currently working toward the Ph.D.~degree in robotics at the University of Toronto Institute for Aerospace Studies (UTIAS). From 2016 to 2021, he was a Guidance Navigation and Controls Engineer with MDA Space, Canada. His research interests include the application of convex optimization in robotics, particularly for certification of state-estimation algorithms. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{_photos/ben-small.jpeg}}]{Ben Agro} received the B.A.Sc.~degree from the University of Toronto in engineering science, specializing in robotics, in 2023, from the University of Toronto, Toronto, ON, Canada, where he is currently working toward a Ph.D.~degree in computer science under Prof. Raquel Urtasun. He is a Research Scientist with Waabi, Toronto, Canada, an autonomous trucking company, working on their perception and forecasting systems. His research interests include self-supervised methods and representation learning, object detection, trajectory forecasting, and occupancy forecasting.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{_photos/tim.jpg}}]{Timothy D. Barfoot} (Fellow, IEEE) received the B.A.Sc.~degree in engineering science and the Ph.D.~degree in aerospace science and engineering from University of Toronto, Toronto, ON, Canada, in 1997 and 2002, respectively. He is currently a Professor with the Robotics Institute, University of Toronto. He works in the areas of guidance, navigation, and control of autonomous systems for a variety of applications. His research interests include developing methods to allow robotic systems to operate over long periods of time in large-scale, unstructured, three-dimensional environments, using rich onboard sensing (e.g., cameras and laser rangefinders) and computation.
\end{IEEEbiography}

